Cross-Lingual Transfer Robustness to Lower-Resource Languages on Adversarial Datasets

Multilingual Language Models (MLLMs) exhibit robust cross-lingual transfer capabilities, or the ability to leverage information acquired in a source language and apply it to a target language. These capabilities find practical applications in well-established Natural Language Processing (NLP) tasks such as Named Entity Recognition (NER). This study aims to investigate the effectiveness of a source language when applied to a target language, particularly in the context of perturbing the input test set. We evaluate on 13 pairs of languages, each including one high-resource language (HRL) and one low-resource language (LRL) with a geographic, genetic, or borrowing relationship. We evaluate two well-known MLLMs--MBERT and XLM-R--on these pairs, in native LRL and cross-lingual transfer settings, in two tasks, under a set of different perturbations. Our findings indicate that NER cross-lingual transfer depends largely on the overlap of entity chunks. If a source and target language have more entities in common, the transfer ability is stronger. Models using cross-lingual transfer also appear to be somewhat more robust to certain perturbations of the input, perhaps indicating an ability to leverage stronger representations derived from the HRL. Our research provides valuable insights into cross-lingual transfer and its implications for NLP applications, and underscores the need to consider linguistic nuances and potential limitations when employing MLLMs across distinct languages.

==> review.tex <==
#clarification on figures and tables #1:
> "The three pairs involving Spanish (Spanish/Aragonese, Spanish/Asturian, and Spanish/Catalan) are notable here, in that P5 brings the native model down to the performance level of the unperturbed cross-lingual transfer model" In Figure 2, the languages are only shown for some data points, and not for any of the native models, and so it was unclear how to verify this claim from the information in the figure.

    It is important to note that Figure 2 only shows change in F1 after perturbation, and is therefore the wrong place to be looking for confirmation that P5 brings the native models down to the level of the cross-lingual transfer (as Figure 2 does not show raw performance). Rather, the numbers on which we base that conclusion are found in Table 5. For example, under P5, native Catalan NER performance is 86.5 F1 while unperturbed Spanish-Catalan NER performance is 85.1. The numbers concerning Asturian and Aragonese are more extreme, which is the basis for this assertion.  Table 5 has a lot of numbers, so we can nonetheless see how this was missed.  In the final copy, we will bold or otherwise indicate the numbers in Table 5 that are the subject of further discussion later, and indicate this in the table caption.  We will also add a reference to Table 5 in the paragraph you singled out above to make clear where this information lies.
    
#clarification on figures and tables #2:
> Elements of the discussion of results in Section 6 were similarly difficult to follow: "We can see that using an HRL→LRL transfer setting never reaches the performance of the native LRL fine-tuning, falling below by ∼1-30% F1/accuracy." The F1 and accuracy for native LRL fine-tuning do not appear to be reported.

    These are reported in Table  5 in the Base column.  Native LRL numbers are the second row of each dyad (i.e.., where L1 and L2 are the same).

#clarification on figures and tables #3:
> Section 6: "On average, MBERT appears more robust to the perturbations we applied" This average for MBERT (and XLM-R) does not seem to be reported. Including it could help to support this claim.

    While the average can be obtained from the individual numbers in Table 5, understandably a reader will not take the time to do that so we will add these average numbers to Table 5 or Table 6.

#clarification on figures and tables #4:
> Technically Hindi is not a minority language, in fact it is very resource rich compared to other languages of the Indian subcontinent and is the third most spoken language in the world. Hence these terms may not really be applicable to the Arabic Hindi pair- but as the authors state this is the 'control pair'. Nevertheless it might be more explicitly stated as an exception. The vocabulary overlap between Ar-Hi is also negligible.

    This is a control pair precisely because the differing scripts lower the overlap at the token level even when borrowing (in this case mediated via Farsi) may result in vocabulary overlap (you are correct though, that core vocabulary overlap between the two is negligible, although two core Hindi terms—aadmi “man” and aurat “woman”—are of Arabic origin).  We will more explicitly state that this is an exception.  Hindi is resource rich compared to other Indian languages, but comparatively resource poor compared to languages of comparable speaker base size (e.g., English or Spanish).  When we say “LRL” we are speaking in terms of resources available for NLP technology specifically.  If we consider the token counts of different languages for a common corpus like CC-100, we find that there are 55.6M English tokens, 9.3M Spanish tokens, and only 1.72M Hindi tokens—much more comparable to a language like Catalan (at 1.75M tokens) [2].  We’ll make this clear in Section 3.
    [2] Conneau, A., Khandelwal, K., Goyal, N., Chaudhary, V., Wenzek, G., Guzmán, F., ... & Stoyanov, V. (2019). Unsupervised cross-lingual representation learning at scale. arXiv preprint arXiv:1911.02116.

#clarification on figures and tables #5:
Improve clarity around exact overlap calculations between languages.


novelty:
> The paper does not provide particularly novel ideas, but rather confirms previously known limitations of multilingual models for low-resource languages.
    
    Our novelty lies in introducing new methods for generating adversarial datasets, including through perturbations based on distances of representations in the latent space, thus enhancing cross-lingual transfer challenges, and in our explicit focus on minority and low-resourced languages. We also provide a new dataset for performance analysis (which will be released upon publication). Additionally, we believe that both many of the specific languages we examine have not been examined in this way before (largely being treated as individual use cases or not examined as “junior partners” in MLLMs).  For instance [1] focuses on English, German, and Hindi, and [2] focus on 8 widely-spoken languages (English, Arabic, Chinese, French, Japanese, Korean, Russian, Spanish, and Turkish—on NER only).  We examine an even wider-spectrum of languages, most of them low-resource, on two tasks, and we find that they exhibit different behaviors under perturbation.

    [1] Akshay Srinivasan and Sowmya Vajjala. 2023. A multilingual evaluation of ner robust- ness to adversarial inputs. arXiv preprint arXiv:2305.18933.
    [2] Ricardo A Calix, Jj Ben-Joseph, Nina Lopatina, Ryan Ashley, Mona Gogia, George Sieniawski, and Andrea Brennen. 2022. Saisiyat is where it is at! insights into backdoors and debiasing of cross lingual transformers for named entity recognition. In 2022 IEEE International Confer- ence on Big Data (Big Data), pages 2940–2949. IEEE.

#WordNet:
> Not sure why the authors did not use a manually created resource such as WordNet to extract similar words to create the perturbations. Some errors are quite egregious - e.g. the cases in Table 2. 

    We looked into this but there do not exist WordNets for the 21 languages we examined, for instance in Aragonese.  This is to be expected given that the domain in question is low-resource languages. Secondly, WordNets that do exist for the languages of interest are incomplete or very small, lacking a substantial number of words. Thirdly, WordNet synsets do not necessarily cover alternative potential substitutions that would be sensical, without traversing the synset tree quite far from the word of origin.  For instance, instead of saying "I see my sister that day," one could say "I see my mother that day." Similarly, a WordNet-based approach for synonym replacement becomes challenging when dealing with homographs.


generative models:
> Does not explore cutting-edge generative models, focuses only on encoders.

    We took this approach because 1) encoder models typically demand fewer computational resources, allowing us to perform more experiments; 2) their weights and pipelines are usually fully available on platforms like HuggingFace, in contrast to SOTA decoder models such as GPTs, meaning that we can directly access the embedding spaces to inform our perturbation techniques; 3) most open-weight generative models (e.g., LLaMA 2) are not multilingual; those that are remain closed, such as Chat-GPT.  However, since our techniques are general, we proposed exploring multilingual generative models for future works. An open-source multilingual generative model like XGLM would be potentially suitable for exploration, but we should note that it does not include all the languages we study here, which further indicates a resource deficiency for many languages when it comes to SOTA generative NLP.

#Intro and related work #1:
> Second, the introductory and related work sections could be made much more compact and easier to read. The experiments focus on the problem of the 'unseen' vocabulary items, especially in the context of multilingual language models, but the summarization of related work is very scattered.

    We can condense the intro and make related work more concise.

#Intro and related work #2:
> Shorten lengthy explanation of related work to allow more space for novel contributions.


#Intro and related work #3:
> Have the authors looked at some of the literature on cognates and cross lingual transfer ? 
    
    Yes, for example [1].  They use semantic similarity techniques similar to the ones we use here and demonstrate that for related languages (in this case, Bengali and Assamese), a monolingual model specifically trained for the lower-resourced language can be used to augment MLLM performance in that language, but only where there is word/token overlap with the better-resourced language. They do not examine perturbations like we do.


    [1] Nath, A., Ghosh, R., & Krishnaswamy, N. (2022, October). Phonetic, semantic, and articulatory features in assamese-bengali cognate detection. In Proceedings of the Ninth Workshop on NLP for Similar Languages, Varieties and Dialects (pp. 41-53).


Appendix: expand analysis:
> Expand analysis of particular language pairs that showed noteworthy behaviors.

    Given the inability to submit an appendix to this year's COLING, some of this detail had to be but we will include it in the camera ready version given the extra page

human evaluation:
> Incorporate human evaluation for tasks beyond metrics to assess quality and relevance of perturbations.

    We sourced a qualitative analysis for Farsi (Section 7.2) but don't have access to native speakers of all the languages in question, as many of them are minority languages with smaller speaker bases.



monolingual models:
> Provide more direct comparison to monolingual models as an alternative approach for low-resource languages.

    Now that we have demonstrated the effect of perturbations on MLLMs, this is a relevant items of future work.  Perhaps monolingual models are more robust to these perturbations, as they have displayed increased task performance on the target languages compared to monolingual models. This is conjectured or demonstrated in some of the examples mentioned in future work [5–8].
    [5] Antti Virtanen, Jenna Kanerva, Rami Ilo, Jouni Luoma, Juhani Luotolahti, Tapio Salakoski, Filip Ginter, and Sampo Pyysalo. 2019. Multilingual is not enough: Bert for finnish. arXiv preprint arXiv:1912.07076.
    [6] Raphael Scheible, Fabian Thomczyk, Patric Tippmann, Victor Jaravine, and Martin Boeker. 2020. Gottbert: a pure german language model. arXiv preprint arXiv:2012.02110.
    [7] Hasan Tanvir, Claudia Kittask, Sandra Eiche, and Kairit Sirts. 2021. Estbert: A pretrained language-specific bert for estonian. In Proceedings of the 23rd Nordic Conference on Compu- tational Linguistics (NoDaLiDa), pages 11–19.
    [8] Nath, A., Ghosh, R., & Krishnaswamy, N. (2022, October). Phonetic, semantic, and articulatory features in assamese-bengali cognate detection. In Proceedings of the Ninth Workshop on NLP for Similar Languages, Varieties and Dialects (pp. 41-53).

odd similaritis #1:
> Further analyze the effect of embedding similarities driving odd semantic substitutions in perturbations.

    This is also a good idea, given that the pertinence of perturbation to LRL language models has been established, and could potentially be correlated to factors of the training data or regime.

odd similaritis #2:
> One way to make sure that the cosine similarity substitutions make sense, perhaps some manual sampling of the substituted words could be made for all pairs. Was this considered ?
    
    This is a good suggestion.  We did consider this and we don’t have access to native speakers of all the languages in question.  For some of those that we do (e.g., Farsi), this type of examination was performed.

Dataset release: 
will the datasets created in the paper be released ?
Yes. Our novel dataset and our experimental code will be released upon publication.

Typos:

Add missing inline citations in Introduction and Related Works sections. 

Fix minor typo in Section 3 when referring to the Reuters Corpus dataset. 

Establish consistent abbreviation format for low/high resource language (LRL/HRL).

Perturbation: randomless -> randomness

(page 6): repeated "changes from"

please also cite the source of the models bert-base-multilingual-cased and xlm-roberts-base.


Main Body Checklist:
clarification on figures and tables #1: Done
clarification on figures and tables #2: Done
clarification on figures and tables #3: Done
clarification on figures and tables #4: Done
clarification on figures and tables #5: Done
Novelty: Done
WordNet:Done
Generative models: Done
Intro and related work #1: Done
Intro and related work #2: Done
Intro and related work #3: Done
Dataset release: Done
Typos: Done

Appendix Checklist: 
I need to know what should I add regarding the following question:
> Expand analysis of particular language pairs that showed noteworthy behaviors.

    Given the inability to submit an appendix to this year's COLING, some of this detail had to be but we will include it in the camera ready version given the extra page

